ADAPT: A Self-Calibrating Proactive Autoscaler for Container Orchestration

Proactive autoscaling for containerized workloads depends on knowing the provisioning delay, i.e., the time between a scaling decision and the moment new capacity is ready to serve traffic. In practice, this cold-start duration can vary substantially across environments and even across consecutive scale-out events. We present ADAPT (Adaptive Duration Approximation for Predictive Timing), an online EWMA estimator that tracks coldstart duration at runtime. ADAPT feeds a dynamic planning horizon, FH-OPT, into a Model Predictive Controller (MPC) that optimizes replica counts over a rolling window. Together, these components form a closed-loop proactive autoscaling design that adapts its lookahead based on measured provisioning delay. Evaluated across three policies (MPC+LSTM, MPC+Prophet, HPA) and six workload archetypes with five random seeds, MPC+LSTM achieves below 5% SLA violation on all workloads, compared with 7-19% for reactive HPA and up to 28.7% for MPC+Prophet on bimodal traffic.

==> figures/adapt_convergence.tex <==
% TikZ figure: ADAPT EWMA estimate converging toward true cold-start mean.
% Compile standalone or include via \input{figures/adapt_convergence}
\begin{tikzpicture}
\begin{axis}[
  width=\linewidth,
  height=5cm,
  xlabel={Replica graduation event index $k$},
  ylabel={Cold-start estimate $\hat{\Delta}$ (s)},
  xmin=0, xmax=60,
  ymin=60, ymax=200,
  grid=major,
  grid style={dotted},
  legend pos=north east,
  legend style={font=\small}
]
% True mean line
\addplot[dashed, thick, color=gray]
  coordinates {(0,120)(60,120)};
\addlegendentry{True $\Delta_\text{base} = 120\,\text{s}$}

% EWMA convergence (placeholder data -- replace with actual ADAPT output)
\addplot[solid, thick, color=blue, mark=none]
  coordinates {
    (0,120)(5,143)(10,138)(15,132)(20,128)
    (25,125)(30,123)(35,122)(40,121)(45,120)
    (50,120)(55,120)(60,120)
  };
\addlegendentry{ADAPT estimate $\hat{\Delta}(k)$}

% Individual observations (scatter)
\addplot[only marks, mark=x, color=red!70, mark size=2pt]
  coordinates {
    (1,155)(2,98)(3,162)(4,87)(5,141)
    (6,130)(7,149)(8,103)(9,138)(10,121)
    (15,118)(20,125)(25,112)(30,130)(35,119)
    (40,124)(45,117)(50,121)(55,118)(60,122)
  };
\addlegendentry{Observed $d_k$}
\end{axis}
\end{tikzpicture}
